Optimizing Curbside Parking Resources Subject to Congestion Constraints

To gain theoretical insight into the relationship between parking scarcity and congestion, we describe block-faces of curbside parking as a network of queues. Due to the nature of this network, canonical queueing network results are not available to us. We present a new kind of queueing network subject to customer rejection due to the lack of available servers. We provide conditions for such networks to be stable, a computationally tractable "single node" view of such a network, and show that maximizing the occupancy through price control of such queues, and subject to constraints on the allowable congestion between queues searching for an available server, is a convex optimization problem. We demonstrate an application of this method in the Mission District of San Francisco; our results suggest congestion due to drivers searching for parking stems from an inefficient spatial utilization of parking resources.

==> data.tex <==
\textcolor{red}{add citations}City planners in major urban centers have recently come into a windfall of data; in particular, digital parking meters and parking space sensors have afforded transportation departments and opportunity to comprehensively evaluate the effectiveness of their policies.

Yet, no city has completely implemented full-scale transportation sensor grids
that include active monitoring of parking on a space by space basis. Regardless
whether such a goal may be reached, however, many cities have a growing history
of parking transaction data collected by digital meters. These data can be used
to estimate parking occupancy (i.e.~the proportion of spaces in use at any given time): a common metric used by transportation engineers and urban planners to determine the utilization of parking resources. 

In addition to data maintained by municipalities with respect to the amount and location of parking supply, transaction data provides a estimate of how long a driver intended to park, as well as the total volume of drivers parking at a location on moment to moment basis. Given that a considerable amount of transportation literature is focused on congestion, and the impact parking supply and demand has on congestion, this work aims to relate occupancy levels and resulting congestion resulting from what the literature refers to as \emph{cruising for parking}.

\textcolor{red}{I think this is an important point and should be moved to the
introduction. This highlights why our work is novel and this section feels a bit
misnamed given we aren't really talking about data per se but rather laying the
background or setup for why what we are doing is important}.
There are then two components to our problem: 1) block-faces with on-street
parking are servicing cars at a rate which is approximately observed in
transaction data and 2) people unable to find parking are bound to surface
street topology in their search. The former can be modeled by a queue, and the
latter can be expressed as a graph or network. We therefore develop a queue network model that tries to recover the \emph{arrival rate} of drivers that can achieve an observed occupancy and estimate the resulting \emph{congestion} along network edges due to the probability of any queues being full. To our surprise, little research in general queuing networks has fallen into a service regime we describe in section \ref{sec:model}.


==> gradient.tex <==
% \label{sec:gradient}
%
% %log barrier
% %We apply the chain rule to $(g \circ f \circ \mathcal{U})(p)$, giving us
%
% %\begin{equation}\label{eqn:grad}
% % \frac{dx}{dp} = \frac{dg(y)}{dy} \cdot \frac{dy}{du} %\cdot \frac{du}{dp}
% %\end{equation}.
%
% %The derivative of the first term in equation \ref{eqn:grad} is, in terms of $\pi_k$,
%
% %\begin{equation}
% % \frac{dg(y)}{dy} = \pi_k + (\frac{d}{dy} \cdot \pi_k)y
% %\end{equation},
%
% %while the second and third terms of equation \ref{eqn:grad} are given by equations \ref{eqn:firstderiv} and the elasticities of each blockface $-\alpha$, respectively. Since we can write the gradient \ref{eqn:grad} explicitly, the optimization problem \ref{eqn:opt} can be solved by minimizing $(g \circ f \circ \mathcal{U})(p)$ with the log barrier method.
%
% %This is convenient because any convex, non-increasing elasticity function can be applied; as yet, only estimates of price elasticity exist for a small number of cities and given further study, a representative convex function of price elasticity could exist, and easily be applied in this context.
%
% %\begin{equation}\label{eqn:opt_log}
% %\begin{aligned}
% %& \underset{p}{\text{minimize}}
% %& & -g(f(\mathcal{U}(p))) - \mu \sum_{n=1}^{m} \phi \\
% %& \text{subject to}
% %& & g_i(p_i) \leq \bar{x}_i, \; i = 1, \ldots, m.
% %\end{aligned}
% %\end{equation}
%
% %but this would lead to an unnecessary body of calculations. Because each block-face is essentially decoupled with respect to the traffic it generates (regardless of the proportion of exogenous or endogenous arrivals, the resulting rate of rejection is our constraint value), we instead perform a subgradient descent with a binary penalty function once a block-face's resulting traffic's constraint is met.
%
% %projected gradient descent
% %We use projected gradient descent to solve the optimization problem
% %\eqref{eqn:opt} (see Algorithm~\ref{alg:proj}).
%
% Since \eqref{eqn:opt} is convex, there exist many ways to solve it. We use a projected gradient for the case study in the next section.
% , let $\mathcal{C}$ denote the feasible solution region, and
% $\Proj_{\mathcal{C}}(p)$ be the projection of a price $p$ onto the feasible
% solution region. Because occupancies at each block-face are orthogonal with
% respect to price, the gradient $\mc{U}(p)$ always points in the directions of the elasticities at each block-face.
%
% Algorithm~\ref{alg:proj} contains the psuedocode for the projected gradient
% descent scheme we use to solve \eqref{eqn:opt}.
%
% \begin{algorithm}
% 	\KwData{block-face elasticities $\nabla\mathcal{U}(\bm{p}) = \bm{\alpha}$, number of spaces $k_i$ at each block-face, and maximum allowable traffic $\bar{\bm{x}}$.}
% 	\KwResult{Maximum occupancy $\bm{u}$ subject to block-face traffic constraints}
% 	tolerance: $\epsilon$\;
% 	initialize price: $\bm{p}^{(0)},$\;
% 	step size: $\beta = 1, \gamma \in (0,1)$\;
% 	\While{$||\bm{p}^{(t)} - \bm{p}^{(t - 1)}||^{2}_{2} > \epsilon$}{
% 		update p\;
% 		$\bm{p}^{(t+1)} = \bm{p}^{(t)} - \beta \nabla \mathcal{U}(\bm{p}^{\bm{t}})$\;
% 		adaptively choose new step size in projected space\;
% 		\While{$\Proj_{\mathcal{C}}(\mathcal{U}(\bm{p^{(t+1)}} - \beta \nabla
%         \mathcal{U}(\bm{p}^{(t+1)}))) > \Proj_{\mathcal{C}}(\mathcal{U}(\bm{p}^{(t+1)}) - \frac{\beta}{2} ||\nabla \mathcal{U}(\bm{p}^{(t+1)})||^{2}_{2})$}{
% 			$\beta = \gamma \beta$\;
% 		}
% 	}
% 	\caption{Projected gradient descent to minimize $-\mathcal{U}(p)$ subject to congestion constraints.}
%     \label{alg:proj}
% \end{algorithm}

